Small Logic-based Multipliers with Incomplete Sub-Multipliers for FPGAs

There is a recent trend in artificial intelligence (AI) inference towards lower precision data formats down to 8 bits and less. As multiplication is the most complex operation in typical inference tasks, there is a large demand for efficient small multipliers. The large DSP blocks have limitations implementing many small multipliers efficiently. Hence, this work proposes a solution for better logic-based multipliers that is especially beneficial for small multipliers. Our work is based on the multiplier tiling method in which a multiplier is designed out of several sub-multiplier tiles. The key observation we made is that these sub-multipliers do not necessarily have to perform a complete (rectangular) NxK multiplication and more efficient sub-multipliers are possible that are incomplete (non-rectangular). This proposal first seeks to identify efficient incomplete irregular sub-multipliers and then demonstrates improvements over state-of-the-art designs. It is shown that optimal solutions can be found using integer linear programming (ILP), which are evaluated in FPGA synthesis experiments.

==> figs/table_synth_prev_inferred.tex <==
\begin{table*}[t]
\centering
    \caption{Comparison to previous tiling and inferred multiplier}     
    \label{tb:impr_prev_tiling}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}
{lr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}
\toprule
 y\textbackslash x&\multicolumn{3}{c}{1}&\multicolumn{3}{c}{2}&\multicolumn{3}{c}{3}&\multicolumn{3}{c}{4}&\multicolumn{3}{c}{5}&\multicolumn{3}{c}{6}&\multicolumn{3}{c}{7}&\multicolumn{3}{c}{8}&\multicolumn{3}{c}{9}&\multicolumn{3}{c}{10}&\multicolumn{3}{c}{11}&\multicolumn{3}{c}{12}&\multicolumn{3}{c}{13}&\multicolumn{3}{c}{14}&\multicolumn{3}{c}{15}&\multicolumn{3}{c}{16}\\ 
 \hline
1&1&0\%&0\%&1&0\%&0\%&2&0\%&0\%&2&0\%&0\%&3&0\%&0\%&3&0\%&0\%&4&0\%&0\%&4&0\%&0\%&5&0\%&0\%&5&0\%&0\%&6&0\%&0\%&6&0\%&0\%&7&0\%&0\%&7&0\%&0\%&8&0\%&0\%&8&0\%&0\%\\
2&1&0\%&0\%&2&0\%&0\%&3&0\%&0\%&5&0\%&0\%&6&0\%&0\%&7&0\%&0\%&8&0\%&0\%&9&0\%&0\%&10&0\%&0\%&11&0\%&0\%&12&0\%&0\%&13&0\%&0\%&14&0\%&0\%&15&0\%&0\%&16&0\%&0\%&17&0\%&0\%\\
3&2&0\%&0\%&3&0\%&0\%&5&0\%&0\%&9&10.0\%&10.0\%&12&0\%&7.6\%&14&6.6\%&6.6\%&16&5.8\%&5.8\%&18&5.2\%&10.0\%&21&0\%&4.5\%&23&4.1\%&8.0\%&25&7.4\%&7.4\%&28&0\%&6.6\%&30&3.2\%&6.2\%&32&3.0\%&8.5\%&34&2.8\%&8.1\%&37&2.6\%&7.5\%\\
4&2&0\%&0\%&5&0\%&0\%&10&0\%&0\%&12&7.6\%&25.0\%&14&17.6\%&33.3\%&17&10.5\%&34.6\%&20&9.0\%&31.0\%&23&11.5\%&32.3\%&26&10.3\%&31.5\%&28&12.5\%&31.7\%&31&11.4\%&29.5\%&34&10.5\%&29.1\%&37&9.7\%&28.8\%&39&11.3\%&30.3\%&42&10.6\%&30.0\%&45&10.0\%&29.6\%\\
5&3&0\%&0\%&6&0\%&0\%&12&0\%&7.6\%&15&11.7\%&28.5\%&18&10.0\%&18.1\%&22&0\%&15.3\%&27&3.5\%&12.9\%&31&0\%&11.4\%&34&2.8\%&15.0\%&38&2.5\%&13.6\%&41&2.3\%&16.3\%&46&0\%&13.2\%&49&0\%&15.5\%&52&1.8\%&16.1\%&56&0\%&16.4\%&60&0\%&15.4\%\\
6&3&0\%&0\%&7&0\%&0\%&14&6.6\%&6.6\%&17&0\%&34.6\%&22&0\%&15.3\%&27&0\%&27.0\%&34&0\%&19.0\%&38&0\%&20.8\%&42&0\%&22.2\%&46&0\%&25.8\%&50&0\%&26.4\%&54&0\%&27.0\%&58&0\%&27.5\%&62&0\%&27.9\%&66&0\%&28.2\%&70&0\%&28.5\%\\
7&4&0\%&0\%&8&0\%&0\%&16&5.8\%&5.8\%&20&9.0\%&31.0\%&27&3.5\%&12.9\%&34&0\%&19.0\%&36&12.1\%&29.4\%&42&10.6\%&27.5\%&47&7.8\%&28.7\%&52&8.7\%&32.4\%&58&6.4\%&30.9\%&63&7.3\%&31.5\%&68&8.1\%&31.3\%&73&7.5\%&31.7\%&78&8.2\%&31.5\%&83&6.7\%&31.9\%\\
8&4&0\%&0\%&9&0\%&0\%&19&0\%&5.0\%&23&11.5\%&32.3\%&30&3.2\%&14.2\%&38&0\%&20.8\%&42&10.6\%&27.5\%&48&7.6\%&31.4\%&54&8.4\%&30.7\%&61&6.1\%&31.4\%&68&4.2\%&30.6\%&73&5.1\%&31.1\%&80&2.4\%&30.4\%&85&4.4\%&30.8\%&91&5.2\%&31.0\%&98&2.0\%&30.4\%\\
9&5&0\%&0\%&10&0\%&0\%&21&0\%&4.5\%&26&10.3\%&31.5\%&36&-2.8\%&10.0\%&42&0\%&22.2\%&47&6.0\%&28.7\%&54&10.0\%&30.7\%&61&7.5\%&23.7\%&68&6.8\%&22.7\%&75&6.2\%&21.8\%&81&5.8\%&22.8\%&88&4.3\%&22.1\%&95&5.0\%&22.1\%&101&4.7\%&22.3\%&108&5.2\%&22.3\%\\
10&5&0\%&0\%&11&0\%&0\%&23&4.1\%&8.0\%&28&12.5\%&31.7\%&38&2.5\%&13.6\%&46&0\%&25.8\%&52&10.3\%&32.4\%&61&6.1\%&31.4\%&69&5.4\%&21.5\%&75&8.5\%&36.9\%&83&6.7\%&36.6\%&90&6.2\%&37.0\%&98&4.8\%&36.7\%&106&3.6\%&37.2\%&114&2.5\%&36.3\%&122&1.6\%&36.7\%\\
11&6&0\%&0\%&12&0\%&0\%&25&3.8\%&7.4\%&31&11.4\%&29.5\%&41&2.3\%&16.3\%&50&0\%&26.4\%&59&4.8\%&29.7\%&67&5.6\%&31.6\%&75&6.2\%&21.8\%&83&6.7\%&36.6\%&92&8.9\%&23.9\%&101&7.3\%&22.9\%&109&7.6\%&23.2\%&117&7.1\%&23.0\%&126&5.2\%&22.6\%&134&5.6\%&22.5\%\\
12&6&0\%&0\%&13&0\%&0\%&28&0\%&6.6\%&34&10.5\%&29.1\%&46&0\%&13.2\%&54&0\%&27.0\%&63&8.6\%&31.5\%&73&6.4\%&31.1\%&81&5.8\%&22.8\%&90&6.2\%&37.0\%&101&6.4\%&22.9\%&110&6.7\%&34.9\%&120&4.0\%&34.0\%&128&3.7\%&34.3\%&137&4.1\%&34.4\%&146&4.5\%&33.6\%\\
13&7&0\%&0\%&14&0\%&0\%&30&3.2\%&6.2\%&37&9.7\%&28.8\%&49&2.0\%&15.5\%&58&0\%&27.5\%&69&6.7\%&30.3\%&79&3.6\%&31.3\%&89&4.3\%&21.2\%&98&4.8\%&36.7\%&109&6.8\%&23.2\%&119&7.0\%&34.6\%&129&6.5\%&27.1\%&139&4.7\%&27.2\%&151&3.8\%&25.9\%&159&4.2\%&27.0\%\\
14&7&0\%&0\%&15&0\%&0\%&32&3.0\%&8.5\%&39&11.3\%&30.3\%&52&1.8\%&16.1\%&62&0\%&27.9\%&73&8.7\%&31.7\%&85&4.4\%&30.8\%&94&6.0\%&22.9\%&106&3.6\%&37.2\%&117&5.6\%&23.0\%&128&5.1\%&34.3\%&139&4.7\%&27.2\%&151&4.4\%&34.9\%&163&2.9\%&33.7\%&173&2.8\%&33.7\%\\
15&8&0\%&0\%&16&0\%&0\%&34&2.8\%&8.1\%&42&10.6\%&30.0\%&56&1.7\%&16.4\%&66&0\%&28.2\%&78&7.1\%&31.5\%&92&3.1\%&30.3\%&102&3.7\%&21.5\%&114&2.5\%&36.3\%&127&5.2\%&22.0\%&137&4.1\%&34.4\%&150&4.4\%&26.4\%&162&3.5\%&34.1\%&174&5.9\%&22.3\%&187&3.1\%&22.0\%\\
16&8&0\%&0\%&17&0\%&0\%&37&2.6\%&7.5\%&45&10.0\%&29.6\%&60&0\%&15.4\%&70&0\%&28.5\%&84&6.6\%&31.1\%&97&3.0\%&31.2\%&108&4.4\%&22.3\%&122&1.6\%&36.7\%&134&4.9\%&22.5\%&146&3.9\%&33.6\%&159&4.7\%&27.0\%&174&1.6\%&33.3\%&186&4.1\%&22.5\%&199&2.9\%&34.1\%\\


\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}







\begin{table*}[t]
\centering
    \caption{Comparison to previous truncated tiling}     
    \label{tb:impr_prev_tiling_trunc}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}
{lr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}cr@{\hspace{0.1cm}}c}
\toprule
 y=x&\multicolumn{2}{c}{1}&\multicolumn{2}{c}{2}&\multicolumn{2}{c}{3}&\multicolumn{2}{c}{4}&\multicolumn{2}{c}{5}&\multicolumn{2}{c}{6}&\multicolumn{2}{c}{7}&\multicolumn{2}{c}{8}&\multicolumn{2}{c}{9}&\multicolumn{2}{c}{10}&\multicolumn{2}{c}{11}&\multicolumn{2}{c}{12}&\multicolumn{2}{c}{13}&\multicolumn{2}{c}{14}&\multicolumn{2}{c}{15}&\multicolumn{2}{c}{16}\\ 
 \hline
&1& 0\%&1& 0\%&3& 57.142\%&10& -11.111\%&15& 11.764\%&22& 0\%&28& 12.500\%&37& 7.500\%&48& 5.882\%&57& 14.925\%&68& 12.820\%&80& 10.112\%&96& 7.692\%&111& 8.264\%&127& 2.307\%&144& 2.702\%\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}
